Turbulence Dissipation and Particle Injection in Non-Linear Diffusive Shock Acceleration with Magnetic Field Amplification

The highly amplified magnetic fields suggested by observations of some supernova remnant (SNR) shells are most likely an intrinsic part of efficient particle acceleration by shocks. This strong turbulence, which may result from cosmic ray driven instabilities, both resonant and non-resonant, in the shock precursor, is certain to play a critical role in self-consistent, nonlinear models of strong, cosmic ray modified shocks. Here we present a Monte Carlo model of nonlinear diffusive shock acceleration (DSA) accounting for magnetic field amplification through resonant instabilities induced by accelerated particles, and including the effects of dissipation of turbulence upstream of a shock and the subsequent precursor plasma heating. Feedback effects between the plasma heating due to turbulence dissipation and particle injection are strong, adding to the nonlinear nature of efficient DSA. Describing the turbulence damping in a parameterized way, we reach two important results: first, for conditions typical of supernova remnant shocks, even a small amount of dissipated turbulence energy (~10%) is sufficient to significantly heat the precursor plasma, and second, the heating upstream of the shock leads to an increase in the injection of thermal particles at the subshock by a factor of several. In our results, the response of the non-linear shock structure to the boost in particle injection prevented the efficiency of particle acceleration and magnetic field amplification from increasing. We argue, however, that more advanced (possibly, non-resonant) models of turbulence generation and dissipation may lead to a scenario in which particle injection boost due to turbulence dissipation results in more efficient acceleration and even stronger amplified magnetic fields than without the dissipation.

==> response <==
We would like to thank the referee again for the very careful review of our paper and for spotting the inconsistensies that we missed. Our responses to the comments are below:

***

COMMENT: Page 21 of the new version, last paragraph: there is a small discrepancy between the numbers reported here and those actually reported in Table 2. Please correct it.

RESPONSE: We corrected the numbers.

***

COMMENT: Page 23, first period: at the end of the period the reference should be to Figure 1.

RESPONSE: We fixed the reference.

***

COMMENT: Page 29, in the third paragraph of the Conclusion section mention could be added to the fact that for the time being $p_{max}$ is found to actually decrease with increasing $\alpha_H$ (due to the decreasing strength of the amplified field), since later in the section the authors speculate on the possibility that cascading phenomena could lead to reverse this trend.

RESPONSE: By "population of the high energy particles is not much changed" we meant, of course, the shape and the normalization of the high energy particles below the highest momentum. We added the note that the maximum momentum decreased with the reduction in the effective magnetic field.

***

COMMENT: Page 32, Eq.(A3): in my initial report I was not wondering about the difference in cell-size between PIC and Hybrid PIC simulations, but rather about the size of the simulation box, which for Hybrid PIC is here defined as the gyroradius of the highest energy particles while for PIC it was defined in terms of their diffusion length, $~(c/u_0)$ times larger.

RESPONSE: Equation (A3) provided "the most optimistic estimate" for the number of cells. But we agree with the comment: for consistency it is better to define the size of the simulation box in both cases as one diffusion length of the highest energy particles. We made a number of changes in equations (A1) - (A4) in order to make them consistent with each other for a fair comparison. 

***

COMMENT: Page 41, Eq.(D10): from (D6) one obtains:
\begin{equation}
r_{tot}=\frac{B-\sqrt{B^2-4AC(1-q_{esc})}}{2C(1-q_{esc})}
\end{equation}
 
RESPONSE: This expression is equivalent to the expression in the paper (except for the choice of the sign before the radical). The two solutions of (D6) can be written as 
\begin{equation}
r_{tot}=\frac{B \pm \sqrt{B^2 - 4AC(1-q_{esc})}}{2C(1-q_{esc})}
\end{equation}
as well as
\begin{equation}
r_{tot}=\frac{2A}{B \mp \sqrt{B^2 - 4AC(1-q_{esc})}}.
\end{equation}
The equivalence of these expressions can be verified by multiplying the enumerator and the denominator of the latter expression by $(B \pm \sqrt{B^2 - 4AC(1-q_{esc})})$ and simplifying.


***

In addition to the above corrections, we also made the following changes:

a) in the top panels of Figure 3 we changed the label from "u(x), cm" to "u(x)/u_0" -- the former was a mistake;

b) made a number of minor changes in Appendix A starting from the paragraph containing equations (A1) and (A2). These changes mostly affect the wording and the layout of the estimates (A1) - (A4);

c) on page 10, we added a sentence to the end of the paragraph containing equation (12) for clarity.

